Improving Redundancy Availability: Dynamic Subtasks Modulation for Robots with Redundancy Insufficiency

This work presents an approach for robots to suitably carry out complex applications characterized by the presence of multiple additional constraints or subtasks (e.g. obstacle and self-collision avoidance) but subject to redundancy insufficiency. The proposed approach, based on a novel subtask merging strategy, enforces all subtasks in due course by dynamically modulating a virtual secondary task, where the task status and soft priority are incorporated to improve the overall efficiency of redundancy resolution. The proposed approach greatly improves the redundancy availability by unitizing and deploying subtasks in a fine-grained and compact manner. We build up our control framework on the null space projection, which guarantees the execution of subtasks does not interfere with the primary task. Experimental results on two case studies are presented to show the performance of our approach.

==> experiment/_experiment.tex <==
% This section presents the study of redundancy resolution subject to redundancy insufficiency, and details on how we model them under our control framework.
% \vspace{0.2cm}

% \noindent\textbf{Experimental Cases }: As illustrated in Fig.~\ref{fig1:subfig:human}, this study is about a mobile robot serving a cup of tea. In this process, when a pedestrian passes by, the platform of the robot needs to avoid the pedestrian, and the end effector should keep the tea at a desired pose. 

% In this process, when a human walks by, the robot needs to avoid the pedestrian, and the end effector should keep the tea at a desired pose. 




% (1) Under the general null-space framework (Eq.~\ref{eq:controlLaw_0}) , the robot handles both serving tea and obstacle avoidance tasks at the same time. However, the serving tea task requires 6 DOF, and the obstacle avoidance task requires 3 DOF, so that the robot's DOF are completely used up.
% There are no redundant DOF that can be used in other constraint tasks that may occur, such as joint collision constraints. We will verify whether other constraint issues will arise and how the robot will perform under this traditional method when the conflict occurs.

% (2) Under the Multi-task merging framework (Eq.~\ref{eq:controlLaw_1}) , the robot with insufficiency DOF also needs to handle the tasks of tea serving end, obstacle avoidance, and self-body collision. We will verify how these tasks are time-sharing regulated，as well as the change of weight matrix and its convergence.

% In the comparison experiments, there are actually three tasks. In both control frameworks, we regard the tea serving as the main task, and the obstacle avoidance and the self-body collision avoidance as the secondary subtasks. The above three tasks are generated as follows。




% \textit{
% (1) Under the general null-space framework (Eq.~\ref{eq:controlLaw_0}) , the robot handles both serving tea and obstacle avoidance tasks at the same time. However, the serving tea task requires 6 DOF, and the obstacle avoidance task requires 3 DOF, so that the robot's DOF are completely used up.
% There are no redundant DOF that can be used in other constraint tasks that may occur, such as joint collision constraints. We will verify whether other constraint issues will arise and how the robot will perform under this traditional method when the conflict occurs.

% (2) Under the Multi-task merging framework (Eq.~\ref{eq:controlLaw_1}) , the robot with insufficiency DOF also needs to handle the tasks of tea serving end, obstacle avoidance, and self-body collision. We will verify how these tasks are time-sharing regulated，as well as the change of weight matrix and its convergence.

% In the comparison experiments, there are actually three tasks. In both control frameworks, we regard the tea serving as the main task, and the obstacle avoidance and the self-body collision avoidance as the secondary subtasks. The above three tasks are generated as follows。



% \begin{itemize}  
%     \item  \textit{Main Task - Tea Serving}: 
%     Specifically, the joint configuration $\q$ is denoted as $[q_1, q_2, \dots,q_9]$, where $q_{1\sim3}$ represent the platform position and yaw angle, and $q_{4\sim9}$ represent the manipulator joint angles respectively. Therefore, the primary task of serving tea at a desired position can be expressed as

% \begin{equation}
% \pmb{\dot\x}_1 = \pmb{g}(\pmb{\x})
% \end{equation}

% Where ${\textbf{g}(\cdot)}$ represents the mapping from the current state to the main task. See the detail in Sec.~\ref{subsec:task_definition}.
% \vspace{0.2cm}

%      \item  \textit{Subtask - Platform Obstacle Avoidance}: 
%      The subtask of platform obstacle avoidance involves avoiding potential collisions between the robot platform and the environment (e.g. the walking human). Therefore, the corresponding three elementary subtasks of one-dimensional obstacle avoidance can be expressed as Eq.~\ref{eq:ds} 

% We formulate the desired  speed ${\dot\x}_{sdi} =\text{f}_i(\pmb{\x}_{\text{sr}i})\in \mathbb{R}\quad i=1,2,3$ of obstacle avoidance  via artificial potential and impedance control as
% %
% \begin{equation}
%      M_{\text{obs}}\ddot{x}_{sdi} = (\textit{F}_{\text{obs}}(\pmb{d_i})-D_{\text{obs}}\dot{x}_{sdi})
% \end{equation}
% %
% where ${M_{\text{obs}}}$ and ${D_{\text{obs}}}$ are virtual chassis mass and damp, and ${\textit{F}_{\text{obs}}_{}(\pmb{d_i})}$ is a repulsive force defined over the distance $\pmb{\x}_{\text{sr}i} = \pmb{d_i}$ between the chassis and obstacle.
% \vspace{0.2cm}

%  \item  \textit{Subtask - Self-Body Collision Avoidance}:


% The subtask of self-body collision avoidance mainly involves avoiding  collision between  manipulator and chassis. We enforce this subtask by control the first three manipulator joint ($x_{4\sim6}$ from the base) to a neutral position. Therefore, the  three elementary subtasks can be expressed as ${\dot\x}_{sdi} =\text{f}_i({\x}_{\text{sr}i})\in \mathbb{R}\quad i=4,5,6$.
% We formulate the desired subtask speed $\dot{x}_{sdi}$ through impedance control as
% %
% \begin{equation}
%      M_{\text{self}}\ddot{x}_{sdi} = (\textit{F}_{\text{self}}-D_{\text{self}}\dot{x}_{sdi}),\quad \textit{F}_{\text{self}} = K_{\text{self}}(x_{sdi}-x_{sri})
% \end{equation}
% %
% where $M_{\text{self}}$, $D_{\text{self}}$ and $K_{\text{self}}$  are virtual impedance parameters, and $x_{sri}$ is the desired neutral position. 


% Therefore, for the Traditional null-space framework, we have 
% \begin{equation}
%     \dot{\x_2}= \A\C=\A[{\dot\x}_{sd1},\;  {\dot\x}_{sd2}, \;{\dot\x}_{sd3}]^T
% \end{equation}

% For the Multi-task merging framework, we have
% \begin{equation}
%     \dot{\x_2}= \A\C=\A[{\dot\x}_{sd1},\;  {\dot\x}_{sd2}, \;...,\;{\dot\x}_{sd6}]^T
% \end{equation}
% \end{itemize}

% \vspace{2cm}}



% However, 

% The pedestrian leaves after 15s, and the manipulator is still locked. It can be seen that in an unstructured dynamic environment, the number of sub-tasks that the robot needs to handle is far more than its own
% DOF. If not handled properly, it will severely limit the execution of robot tasks.


% Under the traditional null-space control framework, the control results are shown in the Fig.~\ref{fig4:SelfColli} \mk
% At the 9s, the pedestrian enter the robot's obstacle avoidance sensing range. In the null space of the main task (tea serving), the joints of the robot are adjusted to avoid pedestrians colliding (Fig. ~\ref{fig4:SelfColli} (b)). However, the robot collides with itself at 13s, the manipulator is locked, and the end effector cannot be stabilized in the desired position (the tea serving task is disturbed). The pedestrian leaves after 15s, and the manipulator is still locked. It can be seen that in an unstructured dynamic environment, the number of sub-tasks that the robot needs to handle is far more than its own
% DOF. If not handled properly, it will severely limit the execution of robot tasks.



% Repeat the above experiment under the framework of Multi-task merging. As shown in Fig. ~\ref{fig5:NonSelfColli}, when the pedestrian enters the robot perception area (at 5s), the robot transitions smoothly to the obstacle avoidance task.

% When the obstacle avoidance is over, the robot automatically adjusts the joints away from the areas prone to self-collision (10s-20s). In other words, when obstacle avoidance is no longer needed, the secondary task positions occupied by "obstacle avoidance" are transferred to "self-collision avoidance". So that idle redundancy can be reused.

% Further, let's focus on the change of Multi-Subtask Merging Matrix $ \A(t)$. As shown in the Fig. ~\ref{fig5:WeightMatrix}, the change process of A matrix corresponding to the subtasks in Fig. ~\ref{fig5:NonSelfColli} is shown. The three subgraphs correspond to the three row vectors of  $ \A(t)$ matrix respectively. The dotted lines correspond to the weights of the three subtasks of obstacle avoidance, and the solid lines correspond to the weights of the three subtasks of the self-
% body collision avoidance.


% We will analyze it from the following aspects：
% \begin{itemize}

% \item \textit{Time division multiplexing} 
% In the Fig. ~\ref{fig5:WeightMatrix}, the weights are assigned to the self-collision subtasks corresponding to the solid lines within 0s-5s. The colors of the curves with the highest weights in the three pictures are different at the same time, which means different rows of $ \A(t)$ matrix correspond to different subtasks. This illustrates the same subtask does not occupy multiple redundancy and will not be repeated.\\

% Starting from the 5s, the dotted line rises one after another ，and the obstacle avoidance subtask is started. At this time, the priority of obstacle avoidance is higher than self-collision, and the robot will first deal with the impending external collision. 10s later, when obstacle avoidance is completed, the redundancy it occupies is transition to the self-collision task represented by the dotted line.
% A large number of subtasks can get redundant DOF and be executed at different times, which embodies the idea of Time Division Multiplexing. Compared with the traditional method Fig. ~\ref{fig4:SelfColli}, the obstacle avoidance task with only three DOF can be performed, our proposed method enables more subtasks to be handled.

% \item \textit{Fine-grained} 
% According to the weight of $ \A(t)$, it can be seen that the subtask adjustment is fine-grained, and the obstacle avoidance task does not require three DOF to be performed simultaneously. In the second sub-figure of the Fig. ~\ref{fig5:WeightMatrix}, once a subtask of obstacle avoidance is completed, the redundancy is allocated to the subtask of self-collision avoidance (at 8s). Within 8s to 10s, the fine-grained self-collision subtasks and the fine-grained obstacle avoidance subtasks are executed at the same time. Which means in the process of obstacle avoidance, if the demand for obstacle avoidance is not high, self-collision avoidance will be adjusted using all available space.

% \item \textit{Convergence} 
%  When the subtask is enabled, the weight of the $ \A(t)$ matrix can quickly converge to a new value. The slope of the adjustment is related to the speed of the subtask response and the Amplitude factor \mk of update rate. Most of them will complete a smooth transition within 1s.


==> experiment/figures.tex <==
\begin{figure}[!t]
	\begin{center}	
		\mbox{
			\hspace{-3.5mm}			
			\subfigure[self collision]{{
					\label{fig3:SelfColli}  
					\includegraphics[height=0.36 \columnwidth, angle=0]{ICRA2021/experiment/figures/SelfColli.png}}}	
					}
		\caption{}
		\label{fig1:intro}
	\end{center}
\end{figure}

==> introduction/__latexindent_temp.tex <==
\section{Introduction}
\label{sec:introduction} 
%======================================%======================================%======================================%=================================
%  \noindent {\color{red} By Wednesday (Lipeng) }
% 冗余机器人占大多数  

% Redundant robots have dominated from perspectives (the popularity, dominant population) the robot community by \noindent {\color{red} ...}
Redundant robots have been dominating with growing popularity 
the robotics community in virtue of their increased dexterity, versatility and adaptability~\cite{hanafusa1981analysis,siciliano1990kinematic,chiaverini2016redundant}.
However, except for few highly specialized systems, most redundant robots still underperform due to lack of relatively sufficient redundancies, especially when operating in unstructured or dynamic environments like households or warehouses characterized by the occurrence of multiple additional subtasks.
Take a drink-serving task as illustrated in Fig.~\ref{fig1:intro} for example. Even though the mobile robot is already equipped with nine degrees of freedom (DOF), as the robot carries a tray upright to serve drinks, only three DOFs will be left as redundancies.
However, besides the primary serving task, the robot is frequently confronted with a large number of additional constraints or subtasks, e.g. obstacles, walking humans and singularity avoidance, which may actually require far more redundancies than the remaining ones. That is, the robot may not be able to deal with all subtasks simultaneously due to the lack of redundancies for subtasking.

We focus on the constrained scenario of \textit{redundancy resolution} problems~\cite{maciejewski1985obstacle,nakamura1987task,ficuciello2015variable} like this, where a redundant robot is supposed to carry out a primary task accompanied by multiple additional subtasks \textbf{but} subject to redundancy insufficiency. 

A straightforward engineering way out of the above redundancy dilemma is to introduce more kinematic redundancies into the robot mechanical structure, which apparently is way too expensive to be repeatable. The majority of prior works on redundancy resolution, either via optimization~\cite{khatib1986real,ge2002dynamic,flacco2015discrete} or task augmentation~\cite{sciavicco1988solution,zanchettin2011general,benzaoui2010redundant}, however, are
%baillieul1985kinematic
fundamentally under the premise the robot can provide sufficient redundancies
%for multitasking, 
i.e. all subtasks can be performed simultaneously with required redundancies.% along the primary task during runtime.

Rather, we noticed that in fact not all aforementioned subtasks have to be performed simultaneously or synchronously % with identical priorities 
thanks to task feature and environment characteristics\footnote{It is acknowledged that there exist cases where subtasks need to be performed strictly simultaneously. For such cases, the engineering augmentation as aforementioned is the only solution.}. For example, a whole-course obstacle avoidance subtask can actually be idle during most of the runtime until some obstacle appears within a certain threshold region, and therefore can be deferred from taking redundancy. Such characteristics give rise to the potential of asynchronicity among subtasks, which essentially accommodates most practical robot applications characterized by dynamic and unstructured environments. 
%but rarely unitized by past studied on redundancy resolution.

It leads to a lightweight but effective solution
%, e.g. based on time division multiplexing (TDM) scheme
that the robot can dynamically allocate redundancies to subtasks
%of higher priorities, 
according to some common rules like task urgency, activeness and importance. 
% such that all subtasks can be properly executed along with the \text{primary task}. 
For example in Fig.~\ref{fig1:intro}, as the robot carries out the primary drinking-serving task, if a human moves closer to the robot (Fig.~\ref{fig1:subfig:human}), the subtask of human avoidance is of an increasing and ultimately dominating priority of taking all redundancies, while all other substasks will be temporarily frozen since no more redundancy is available. As the human walks away, the robot will eventually release the (part of) redundancies,
%from the human avoidance subtask
 until some other subtask takes them, e.g. the self-collision avoidance subtask (Fig.~\ref{fig1:subfig:self}). 

 \begin{figure}[!t]
    %\begin{figure}[htbp!]
        \begin{center}	
            \mbox{
                \hspace{-3.5mm}			
                \subfigure[Human avoidance subtask]{
                        \label{fig1:subfig:human}  
                        \includegraphics[height=0.36 \columnwidth, angle=0]{./figures/human.jpg}}
                \subfigure[Self-collision avoidance subtask]{{
                        \label{fig1:subfig:self}  
                        \includegraphics[height=0.36 \columnwidth, angle=0]{./figures/selfco.jpg}}}	
                        }
            \caption{A drink-serving robot dynamically allocates relatively insufficient redundancies to accomplish multiple subtasks while serving drinks. (a) The human avoidance subtask takes redundancies as the human walks close. (b) The self-collision subtask takes redundancies once the human is far away.}
            \label{fig1:intro}
        \end{center}
    \end{figure}

In this work, we borrow ideas from asynchronous time-division multiplexing (ATDM), propose an approach to subtask management for redundant robots subject to redundancy insufficiency. Our approach unfolds as follows: we first unitize all multi-dimensional subtasks to be executed along with the primary task  
into a set of one-dimensional \textit{elementary subtasks}. This step allows us to greatly improve the redundancy availability by deploying subtasks in a more fine-grained and compact manner. We then manage elementary subtasks by fusing them into a virtual multi-dimensional \textit{secondary task} w.r.t. the primary task. 
We propose a novel \text{subtask merging operator} and an efficient updating strategy to dynamically modulate the secondary task in compliance with the \textit{task status} and \textit{soft priority} derived heuristically.
%from the elementary subtasks. 
Based on the approach, all subtasks can be suitably performed in due course.

Our control framework is built upon previous work of task priority based redundancy resolution~\cite{hanafusa1981analysis,maciejewski1985obstacle,nakamura1987task}, which guarantees the low-level tasks executed in the null space do not interfere with the high-level tasks. We integrate our subtask merging strategy into the null space projection technique to derive a general control framework of subtask management for redundant robots subject to redundancy insufficiency. 
In this framework, the primary task is perfectly performed using a number of required DOFs, while all other subtasks are suitably carried out as a virtual dynamic secondary task using the remaining insufficient redundancy, \text{but} without affecting the primary task. 

% The main contribution of this paper is
% ......

% {\color{red}
% The main contribution of this paper is the derivation of a general control framework of subtask management for redundant robots subject to redundancy insufficiency. Based upon the framework we propose a
% novel dynamic subtask merging operator and an efficient update strategy....}

The paper is organized as follows. Sec.~\ref{sec:relatedwork} and~\ref{sec:background} reviews and recapitulates prior related works. Sec.~\ref{sec:method} presents details of our approach to manage multiple subtasks subject to redundancy insufficiency. Sec.~\ref{sec:experiment} introduces two case studies
%followed by 
with experimental results to verify the performance of our approach. Sec.~\ref{sec:conclusion} concludes this paper and our future work.





% obstacle and singularity avoidance~\cite{}
% joint limits avoidance~\cite{}, complaint motion~\cite{} and singularity avoidance~\cite{} in motion planning and control. 






% in some form or another, but there are usually more important and less important aspects such that a hierarchy among the tasks can be established



% effect：
% \begin{itemize}
%     \item The large number of degrees of freedom (DOF) allows to adapt to a variety of environments and several simultaneous objectives.
%     \item The impressive performance of a human being is substantially due to its versatility.
% \end{itemize}




% \input{ICRA2021/related/related}
% \subsection{Contributions}


% we develop a general framework for multiple tasks management with a limited number of redundancies



%a general framework for managing excessive tasks in redundant robot system,

%which is logically based on the ideas of multiple task priorities.

%Two case studies illustrate the effectiveness of the algorithm on a mobile robot.



==> introduction/fig1.tex <==
\begin{figure}[!t]
%\begin{figure}[htbp!]
	\begin{center}	
		\mbox{
			\hspace{-3.5mm}			
			\subfigure[Human avoidance subtask]{
					\label{fig1:subfig:human}  
					\includegraphics[height=0.36 \columnwidth, angle=0]{./figures/human.jpg}}
			\subfigure[Self-collision avoidance subtask]{{
					\label{fig1:subfig:self}  
					\includegraphics[height=0.36 \columnwidth, angle=0]{./figures/selfco.jpg}}}	
					}
		\caption{A drink-serving robot dynamically allocates relatively insufficient redundancies to accomplish multiple subtasks while serving drinks. (a) The human avoidance subtask takes redundancies as the human walks close. (b) The self-collision subtask takes redundancies once the human is far away.}
		\label{fig1:intro}
	\end{center}
\end{figure}

==> useful.tex <==
% \begin{figure}[t!]
% %\begin{figure}[htbp!]
% 	\begin{center}	
% 		\mbox{
% 			\hspace{-3.5mm}			
% 			\subfigure[Initial config.]{{
% 					\label{fig:subfig:1}  
% 					\includegraphics[width=1.12 in, angle=-0]{introduction/2}}}
% 			\hspace{-3mm}
% 			\subfigure[Drilling four holes ]{{
% 					\label{fig:subfig:2}  
% 					\includegraphics[width=1.12 in, angle=-0]{introduction/1}}}
% 			\hspace{-3mm}		
% 			\subfigure[Inserting four legs]{{
% 					\label{fig:subfig:3}  
% 					\includegraphics[width=1.12 in, angle=-0]{introduction/3}}}					
% 		}
		
% 		\mbox{
% 			\hspace{-3.5mm}
% 			\subfigure[Driling four holes]{{
% 					\label{fig:subfig:4}  
% 					\includegraphics[width=1.12 in, angle=-0]{introduction/4}}}
% 			\hspace{-3mm}
% 			\subfigure[Inserting chair back]{{
% 					\label{fig:subfig:5}  
% 					\includegraphics[width=1.12 in, angle=-0]{introduction/5}}}
% 			\hspace{-3mm}					
% 			\subfigure[Task complete]{{
% 					\label{fig:subfig:6}  
% 					\includegraphics[width=1.12 in, angle=-0]{introduction/6}}}
% 		}			
% 		\caption{11 .}
% 		\label{fig:Intro-Assembling}
% 	\end{center}
% \end{figure}


% \begin{figure}[!t]
% 	\centering
% 	\scriptsize
% 	\def\svgwidth{0.98\columnwidth}
% 	\import{problemFormulation/figs/}{forcefulTask.pdf_tex}
% 	\caption{A}
% 	\label{fig:forcefultask}
% \end{figure}


% The top priority task is executed employing all capabilities of the robotic system. The second
% priority task is then applied to the null space of the top priority task. 

% In other words, the task on the second level is
% executed as good as possible without disturbing or interfering with the first level. 

% The task on level three is then executed without disturbing the two higher priority tasks, and
% so forth.


% obstacle avoidance is essential for satisfactory task completion. Current manipulator applications typically involve removal of potential obstacles from the manipulator’s workspace and the use of fixed motion commands. 

% 异步分时复，是一种根据用户实际需要动态分配信道资源的分时复用技术。异步分时复用技术将用户的数据划分为一个个数据单元，不同用户的数据单元仍按照时分的方式来共享信道，但会根据用户需求动态分配时隙，以避免每帧中出现空闲的时隙。另外，在异步分时复用中，每个用户可以通过占用多个时隙来获得更高的传输速率，最高速率可达到电路总的传输能力，即用户占有所有的时隙。




% \begin{algorithm}[t]
% \caption{algorithm caption} %算法的名字
% \hspace*{0.02in} {\bf Input:} %算法的输入， \hspace*{0.02in}用来控制位置，同时利用 \\ 进行换行
% input parameters A, B, C\\
% \hspace*{0.02in} {\bf Output:} %算法的结果输出
% output result
% \begin{algorithmic}[1]
% \State some description % \State 后写一般语句
% \For{condition} % For 语句，需要和EndFor对应
% 　　\State ...
% 　　\If{condition} % If 语句，需要和EndIf对应
% 　　　　\State ...
% 　　\Else
% 　　　　\State ...
% 　　\EndIf
% \EndFor
% \While{condition} % While语句，需要和EndWhile对应
% 　　\State ...
% \EndWhile
% \State \Return result
% \end{algorithmic}
% \end{algorithm}
